Investigating the fluxes and physics potential of LHC neutrino experiments

The initiation of a novel neutrino physics program at the Large Hadron Collider (LHC) and the purpose-built Forward Physics Facility (FPF) proposal have motivated studies exploring the discovery potential of these searches. This requires resolving degeneracies between new predictions and uncertainties in modeling neutrino production in the forward kinematic region. The present work investigates a broad selection of existing predictions for the parent hadron spectra at FASER$\nu$ and the FPF to parameterize expected correlations in the neutrino spectra produced in their decays and to determine the highest achievable precision for their observation based on Fisher information. This allows for setting constraints on various physics processes within and beyond the Standard Model, including neutrino non-standard interactions. We also illustrate how combining multiple neutrino observables could lead to experimental confirmation of the enhanced-strangeness scenario proposed to resolve the cosmic-ray muon puzzle already during the ongoing LHC Run 3.

==> header.tex <==

\RequirePackage[colorlinks=true
,urlcolor=blue
,anchorcolor=blue
,citecolor=blue
,filecolor=blue
,linkcolor=blue
,menucolor=blue
,linktocpage=true
,pdfproducer=medialab
,pdfa=true
]{hyperref}

\usepackage{amsmath,amssymb,amsthm,amsfonts}
\usepackage{graphicx,tabularx}
\usepackage{color}
\usepackage{multirow}
\usepackage{comment}
\usepackage{enumitem}
\usepackage{cleveref}
\usepackage{slashed}
\usepackage[normalem]{ulem}
\usepackage{scalerel}
\usepackage{wrapfig}
\usepackage{cancel}
\usepackage{xcolor}
\usepackage{float}
\usepackage[letterpaper,dvips,hmargin={1in,1in},vmargin={1in,1in}]{geometry}

\setlist[description]{leftmargin=0.3cm}
\setlist[itemize]{leftmargin=0.5cm}

\newcommand{\be}{\begin{equation} \begin{aligned}}
\newcommand{\ee}{\end{aligned} \end{equation}}
\newcommand{\beqa}{\begin{eqnarray}}
\newcommand{\eeqa}{\end{eqnarray}}

\def\figureautorefname~#1\null{Fig.\,#1\null}
\def\tableautorefname~#1\null{Tab.\,#1\null}
\renewcommand{\sectionautorefname}{Sec.}
\renewcommand{\subsectionautorefname}{Sec.}
\def\equationautorefname~#1\null{Eq.\,(#1)\null}

% General symbols
\newcommand{\im}{\mathrm{i}}
\newcommand{\diff}{\mathrm{d}}
\newcommand{\eg}{{e.\,g.}~}
\newcommand{\ie}{{i.\,e.}~}
\newcommand{\equivalent}{\simeq}
\newcommand{\br}{\mathrm{BR}}

% Units
\newcommand{\ev}{\text{eV}}
\newcommand{\kev}{\text{keV}}
\newcommand{\mev}{\text{MeV}}
\newcommand{\gev}{\text{GeV}}
\newcommand{\tev}{\text{TeV}}

\newcommand{\ab}{\text{ab}}
\newcommand{\iab}{\text{ab}^{-1}}
\newcommand{\fb}{\text{fb}}
\newcommand{\ifb}{\text{fb}^{-1}}
\newcommand{\pb}{\text{pb}}
\newcommand{\ipb}{\text{pb}^{-1}}

\newcommand{\nm}{\text{nm}}
\newcommand{\micm}{\mu\text{m}}
\newcommand{\mm}{\text{mm}}
\newcommand{\cm}{\text{cm}}
\newcommand{\m}{\text{m}}
\newcommand{\km}{\text{km}}

\newcommand{\g}{\text{g}}
\newcommand{\kg}{\text{kg}}
\newcommand{\ton}{\text{t}}
\newcommand{\sr}{\text{sr}}
\newcommand{\ns}{\text{ns}}
\newcommand{\hz}{\text{Hz}}

%comments for changes
\RequirePackage[normalem]{ulem} 
\newcommand{\changed}[2]{{\protect\color{red}\sout{#1}}{\protect\color{blue}\uwave{#2}}}

% personalized comments
\newcommand{\Felix}[1]{\textcolor{magenta}{[FK: #1]}}
\definecolor{emeraldgreen}{RGB}{0, 201, 87}
\newcommand{\st}[1]{\textcolor{emeraldgreen}{[ST: #1]}}
\newcommand{\tm}[1]{\textcolor{orange}{[TM: #1]}}
%\newcommand{\Felix}[1]{}
%\newcommand{\jlf}[1]{}

%\newcommand{\rem}[1]{}
\crefname{section}{Sec.}{Secs.}
\crefname{figure}{Fig.}{Figs.}
\crefname{equation}{Eq.}{Eqs.}
\crefname{table}{Table}{Tables}
\crefname{appendix}{Appendix}{Appendices}

% array
\renewcommand{\arraystretch}{1.2}

%Ref Style
\bibliographystyle{utphys}

% space on top/bottom from figures (copied from revtex)
\setcounter{topnumber}{2}
\def\topfraction{1}
\setcounter{bottomnumber}{1}
\def\bottomfraction{1}
\setcounter{totalnumber}{3}
\def\textfraction{0}
\def\floatpagefraction{1}
\setcounter{dbltopnumber}{2}
\def\dbltopfraction{1}
\def\dblfloatpagefraction{1}
